Dependently Sorted Nominal Signatures

We investigate an extension of nominal many-sorted signatures in which abstraction has a form of instantiation, called generalised concretion, as elimination operator (similarly to lambda-calculi). Expressions are then classified using a system of sorts and sort families that respects alpha-conversion (similarly to dependently-typed lambda-calculi) but not allowing names to carry abstraction sorts, thus constituting a first-order dependent sort system. The system can represent forms of judgement and rules of inference of several interesting calculi. We present rules and properties of the system as well as experiments of representation, and discuss how it constitutes a basis on which to build a type theory where raw expressions with alpha-equivalence are given a completely formal treatment.

==> eptcsdata.tex <==
\providecommand{\firstpage}{82}
\providecommand{\publicationstatus}{Chaudhuri, Nantes-Sobrinho (Eds.): International Workshop on Logical\\ Frameworks and Meta-Languages: Theory and Practice (LFMTP 2025) \\
EPTCS 431, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.431.6}{10.4204/EPTCS.431.6}}

